Automated Misconfiguration Repair of Configurable Cyber-Physical Systems with Search: an Industrial Case Study on Elevator Dispatching Algorithms

Real-world Cyber-Physical Systems (CPSs) are usually configurable. Through parameters, it is possible to configure, select or unselect different system functionalities. While this provides high flexibility, it also becomes a source for failures due to misconfigurations. The large number of parameters these systems have and the long test execution time in this context due to the use of simulation-based testing make the manual repair process a cumbersome activity. Subsequently, in this context, automated repairing methods are paramount. In this paper, we propose an approach to automatically repair CPSs' misconfigurations. Our approach is evaluated with an industrial CPS case study from the elevation domain. Experiments with a real building and data obtained from operation suggests that our approach outperforms a baseline algorithm as well as the state of the practice (i.e., manual repair carried out by domain experts).

==> Table_7_1.tex <==
\begin{table*}[ht]
\scriptsize
  \caption{ Summary of the performed statistical test for the performance metrics when comparing the unguided version of the algorithm with the repairing algorithm. An \^{A}$_{12}$ value that is below 0.5 means that the repair algorithm was better than the unguided version. Statistical significance is set at p-value $<$ 0.05.}
  \label{table:Performance_Metrics_Statistical}
  \centering
  %\resizebox{\textwidth}{!}{
  \begin{tabular}{lllllllllllllllll}
\cline{2-15}
 &  \multicolumn{2}{c}{\textbf{AWT}} & \multicolumn{2}{c}{\textbf{LWT}} & \multicolumn{2}{c}{\textbf{\%WT \textgreater 55s}} & \multicolumn{2}{c}{\textbf{ATT}} & \multicolumn{2}{c}{\textbf{LTT}} & \multicolumn{2}{c}{\textbf{\%TT \textgreater 70s}} & \multicolumn{2}{c}{\textbf{HyperVolume}} \\ \hline
\textbf{Hour}  & \textbf{\^{A}$_{12}$} & \textbf{p-value} & \textbf{\^{A}$_{12}$} & \textbf{p-value} & \textbf{\^{A}$_{12}$} & \textbf{p-value} & \textbf{\^{A}$_{12}$} & \textbf{p-value} & \textbf{\^{A}$_{12}$} & \textbf{p-value} & \textbf{\^{A}$_{12}$} & \textbf{p-value} & \textbf{\^{A}$_{12}$} & \textbf{p-value} \\ \hline
1 & 0.47 & 0.8770 & 0.42 & 0.5302 & 0.58 & 0.5617 & 0.44 & 0.6753 & 0.60 & 0.4075 & 0.42 & 0.5423 & 0.49 & 0.9698 \\
2 & 0.49 & 1.0000 & 0.32 & 0.1516 & 0.50 & 1.0000 & 0.28 & 0.0943 & 0.40 & 0.3661 & 0.37 & 0.3226 & 0.39 & 0.4273 \\
3 & 0.44 & 0.7047 & 0.40 & 0.4073 & 0.43 & 0.5947 & 0.33 & 0.1945 & 0.30 & 0.0335 & 0.43 & 0.6217 & 0.35 & 0.2730 \\
4 & 0.39 & 0.4037 & 0.43 & 0.5786 & 0.39 & 0.4252 & 0.35 & 0.2523 & 0.35 & 0.0767 & 0.45 & 0.7321 & 0.29 & 0.1212 \\
5 & 0.40 & 0.4716 & 0.21 & 0.0110 & 0.34 & 0.2404 & 0.36 & 0.2853 & 0.40 & 0.1674 & 0.35 & 0.2532 & 0.20 & 0.0256 \\
6 & 0.34 & 0.2411 & 0.18 & 0.0058 & 0.22 & 0.0340 & 0.24 & 0.0526 & 0.40 & 0.1674 & 0.20 & 0.0220 & 0.14 & 0.0081 \\
7 & 0.25 & 0.0695 & 0.14 & 0.0028 & 0.15 & 0.0080 & 0.24 & 0.0526 & 0.45 & 0.3681 & 0.20 & 0.0220 & 0.11 & 0.0040 \\
8 & 0.37 & 0.3255 & 0.19 & 0.0115 & 0.23 & 0.0403 & 0.24 & 0.0526 & 0.45 & 0.3681 & 0.16 & 0.0094 & 0.18 & 0.0172 \\
9 & 0.37 & 0.3255 & 0.19 & 0.0110 & 0.15 & 0.0087 & 0.25 & 0.0626 & 0.45 & 0.3681 & 0.16 & 0.0094 & 0.15 & 0.0090 \\
10 & 0.39 & 0.4266 & 0.16 & 0.0060 & 0.15 & 0.0087 & 0.15 & 0.0088 & 0.45 & 0.3681 & 0.15 & 0.0086 & 0.15 & 0.0090 \\
11 & 0.41 & 0.5189 & 0.12 & 0.0023 & 0.15 & 0.0087 & 0.15 & 0.0088 & 0.45 & 0.3681 & 0.18 & 0.0167 & 0.10 & 0.0028 \\
12 & 0.41 & 0.5189 & 0.08 & 0.0007 & 0.16 & 0.0098 & 0.15 & 0.0089 & 0.45 & 0.3681 & 0.21 & 0.0277 & 0.08 & 0.0017 \\ \bottomrule
\end{tabular}%}
\end{table*}
